The multifaceted nature of uncertainty in structure-property linkage with crystal plasticity finite element model

Uncertainty quantification (UQ) plays a critical role in verifying and validating forward integrated computational materials engineering (ICME) models. Among numerous ICME models, the crystal plasticity finite element method (CPFEM) is a powerful tool that enables one to assess microstructure-sensitive behaviors and thus, bridge material structure to performance. Nevertheless, given its nature of constitutive model form and the randomness of microstructures, CPFEM is exposed to both aleatory uncertainty (microstructural variability), as well as epistemic uncertainty (parametric and model-form error). Therefore, the observations are often corrupted by the microstructure-induced uncertainty, as well as the ICME approximation and numerical errors. In this work, we highlight several ongoing research topics in UQ, optimization, and machine learning applications for CPFEM to efficiently solve forward and inverse problems.

==> mlmc_schematic.tex <==
% command to draw a labelled cuboid
% #1 : location of lower left point of cuboid
% #2 : label on front face
% #3 : label below cube
\newcommand{\cuboid}[3]{%
    \begin{scope}[shift={#1}, scale=0.5]
        \draw[rounded corners = 0.1pt] (0,2,2) -- (2,2,2) -- (2,0,2) -- (0,0,2) -- (0,2,2) -- (0,2,0) -- (2,2,0) -- (2,0,0) -- (2,0,2) -- (2,2,2) -- (2,2,0);
        \node[anchor=center] at (1.1,1,2) {#2};
        \node[anchor=north] at (1,0,2) {#3};
    \end{scope}
}

% nice arrow head
\tikzset{%
    >={Stealth[length=2mm, width=1.75mm]}
}

\begin{tikzpicture}[
    every path/.style={semithick, line cap=round},
    every node/.style={inner sep=0pt, outer sep=3pt, execute at end node=\strut}
]
\foreach \mesh [count=\i] in {8, 16, 20, 32, 64}{%
    \pgfmathtruncatemacro{\k}{\i - 1}
    \cuboid{(2*\k, 0)}{$\mesh^3$}{$\ell = \k$}
}
\draw[->] (-1,-1.5) -- node[pos=0.5, anchor=north] {$\ell$} ++(10,0) node[anchor=west, outer sep=6pt, yshift=1pt] {mesh resolution};
% \draw (0,0) rectangle (1,1) node[pos=0.525] {$8^3$};
% \draw (2,0) rectangle (3,1) node[pos=0.525] {$16^3$};
% \draw (4,0) rectangle (5,1) node[pos=0.525] {$20^3$};
% \draw (6,0) rectangle (7,1) node[pos=0.525] {$32^3$};
% \draw (8,0) rectangle (9,1) node[pos=0.525] {$64^3$};
% \node[text width=1cm] at (0.525,-0.525) {$L=0$};
% \node[text width=1cm] at (2.525,-0.525) {$L=1$};
% \node[text width=1cm] at (4.525,-0.525) {$L=2$};
% \node[text width=1cm] at (6.525,-0.525) {$L=3$};
% \node[text width=1cm] at (8.525,-0.525) {$L=4$};
% \draw[line width=2pt,->,blue] (-0.5,-1) -- (10,-1) node[anchor=north east] {\textbf{mesh refinement}};
% \draw[line width=2pt,->,blue] (-0.25,-0.25) -- (10,-0.25) node[anchor=north west] {\textbf{mesh refinement}};
% \node[draw] at (0,0) {$64^3$};
% \node[draw] at (2,0) {$32^3$};
\end{tikzpicture}


